Hamiltonian Particle Dynamics in Fusion Plasmas: Orbital Tomography and Spectrum Analysis for Energy and Momentum Transport under Resonant Non-Axisymmetric Perturbations

This thesis investigates the impact of resonant mode-particle interactions on transport and confinement in toroidal fusion plasmas. Using analytical and numerical approaches, we study how intrinsic and externally applied magnetic perturbations affect plasma particles with different kinetic characteristics, focusing on resonant interactions with guiding-center motion. We develop a novel, computationally efficient method based on Action-Angle variables to identify resonance locations and characterize resonances in guiding-center phase space, including the number of islands in resonance chains and the formation of transport barriers. Using the drift center (DC) approximation, we derive analytical expressions for orbital frequencies and the kinetic $q$ factor for large-aspect-ratio (LAR) equilibria. These results provide the conditions for mode-particle resonances, which can strongly influence particle, momentum, and energy transport and, consequently, plasma confinement. The analytical results are validated against numerical simulations, demonstrating an efficient tool for predicting transport barriers and energetic-particle behavior under non-axisymmetric perturbations. We further extend the orbital-frequency analysis from LAR equilibria to numerically reconstructed, realistic equilibria using a computationally efficient, semi-analytical geometrical method applicable to arbitrary unperturbed equilibria. Finally, for the LAR equilibrium, we extend the analysis to time-dependent perturbations and demonstrate the emergence of Arnold diffusion in guiding-center phase space, highlighting the role of the Arnold web in particle transport. Overall, this work advances the understanding of mode-particle resonant interactions and provides computational tools for predicting transport and confinement in realistic fusion configurations.

==> Preamble/preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% Add spaces between paragraphs
%\setlength{\parskip}{0.5em}
% Ragged bottom avoids extra whitespaces between paragraphs
\raggedbottom
% To remove the excess top spacing for enumeration, list and description
%\usepackage{enumitem}
%\setlist[enumerate,itemize,description]{topsep=0em}
\usepackage{amsmath}
\usepackage{import}
\usepackage{siunitx}
\usepackage{empheq}
\usepackage{bm}
\usepackage[greek,english]{babel}
\usepackage[english]{babel}

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section
\usepackage{ulem}

\usepackage{zref-user}
\usepackage[table,xcdraw]{xcolor}
\usepackage{makecell}
\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  %\RequirePackage{helvet}

  % For use with XeLaTeX
  %  \setmainfont[
  %    Path              = ./libertine/opentype/,
  %    Extension         = .otf,
  %    UprightFont = LinLibertine_R,
  %    BoldFont = LinLibertine_RZ, % Linux Libertine O Regular Semibold
  %    ItalicFont = LinLibertine_RI,
  %    BoldItalicFont = LinLibertine_RZI, % Linux Libertine O Regular Semibold Italic
  %  ]
  %  {libertine}
  %  % load font from system font
  %  \newfontfamily\libertinesystemfont{Linux Libertine O}
\fi

% *****************************************************************************
% **************************** Custom Packages ********************************

% ************************* Algorithms and Pseudocode **************************

%\usepackage{algpseudocode}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}


% *********************************** SI Units *********************************
\usepackage{siunitx} % use this package module for SI units


% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

%Add `custombib' in the document class option to use this section
%\ifuseCustomBib
 %  \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib

% If you would like to use biblatex for your reference management, as opposed to the default `natbibpackage` pass the option `custombib` in the document class. Comment out the previous line to make sure you don't load the natbib package. Uncomment the following lines and specify the location of references.bib file
% \RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty]{biblatex}
% \RequirePackage[
%   backend=biber,      % Use Biber for processing
%   style=numeric-comp, % Numeric citation style (compact)
%   sorting=none,       % Sort by citation order
%   maxnames=3,         % Show up to 3 authors
%   minnames=1          % Use "et al." if more than 3 authors
% ]{biblatex}

% \ExecuteBibliographyOptions{url=false,doi=false,isbn=false}

% \usepackage[style=numeric, giveninits=true, maxnames=3, minnames=1, doi=false, isbn=false, url=false]{biblatex}

% % Format year to appear only in parentheses
% \renewbibmacro*{date+extrayear}{\setunit{\addspace}\printtext[parens]{\printdate}}

% % Remove issue number
% \DeclareFieldFormat{number}{}

% % Ensure pages appear properly
% \DeclareFieldFormat{pages}{#1}


% \usepackage[colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
% \renewbibmacro{in:}{}
% % \renewbibmacro*{doi+eprint+url}{%
% %   \printfield{doi}%
% %   \newunit\newblock%
% %   \iffieldundef{doi}{\printfield{url}}{}}


% \addbibresource{References/references.bib}
%     %\RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty, natbib=true]{biblatex}
%     % \bibliography{References/references} 
%     %\bibliography{Chapter1/chapter1}%Location of references.bib only for biblatex

% %\fi

% % changes the default name `Bibliography` -> `References'
% \renewcommand{\bibname}{References}

\RequirePackage[
  backend=biber,
  style=numeric-comp,
  sorting=none,
  maxnames=3, % Show up to 3 authors before using "et al."
  minnames=3  % Ensure at least 3 authors are shown before "et al."
]{biblatex}

\ExecuteBibliographyOptions{url=false,doi=false,isbn=false,eprint=false}

% Ensure author names are formatted as "Last, F. and Last, F."
\DeclareNameAlias{author}{given-family}

% Format year to appear only in parentheses
\renewbibmacro*{date+extrayear}{%
  \setunit{\addspace}%
  \printtext[parens]{\printdate}%
}

% Remove issue number
\DeclareFieldFormat{number}{}

% Ensure pages appear properly without parentheses
\DeclareFieldFormat{pages}{#1}

% Remove "In:" before journal name
\renewbibmacro{in:}{}

\DeclareBibliographyDriver{article}{%
  \sloppy % Allow better line breaking
  \usebibmacro{author}%
  \setunit{\addcomma\space}%
  \usebibmacro{title}%
  \setunit{\addcomma\space}%
  \printfield{journaltitle}% Changed from journal to journaltitle
  \setunit{\addspace}%
  \printfield{volume}%
  \setunit{\addcomma\space}%
  % \printfield{pages}%
  % \setunit{\addspace}%
  \usebibmacro{date}%
  \finentry%
}

\DeclareBibliographyDriver{book}{%
  \sloppy % Allow better line breaking
  \usebibmacro{author}%
  \setunit{\addcomma\space}%
  \printfield{title}%
  \setunit{\addcomma\space}%
  \printlist{publisher}%
  \setunit{\addcomma\space}%
  \usebibmacro{date}%
  \finentry%
}

% Remove any underline formatting (if present)
\DeclareFieldFormat{title}{#1}
\DeclareFieldFormat{journaltitle}{#1}
\DeclareFieldFormat[article]{title}{#1}



\addbibresource{References/references_fixed.bib}

% changes the default name `Bibliography` -> `References'
\renewcommand{\bibname}{References}


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% *********************** Configure Draft Mode **********************************

% Uncomment to disable figures in `draft'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


% ******************************** Todo Notes **********************************
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}
